Parallelizing Linear Transformers with the Delta Rule over Sequence Length

Transformers with linear attention (i.e., linear transformers) and state-space models have recently been suggested as a viable linear-time alternative to transformers with softmax attention. However, these models still underperform transformers especially on tasks that require in-context retrieval. While more expressive variants of linear transformers which replace the additive update in linear transformers with the delta rule (DeltaNet) have been found to be more effective at associative recall, existing algorithms for training such models do not parallelize over sequence length and are thus inefficient to train on modern hardware. This work describes a hardware-efficient algorithm for training linear transformers with the delta rule, which exploits a memory-efficient representation for computing products of Householder matrices. This algorithm allows us to scale up DeltaNet to standard language modeling settings. We train a 1.3B model for 100B tokens and find that it outperforms recent linear-time baselines such as Mamba and GLA in terms of perplexity and zero-shot performance on downstream tasks. We also experiment with two hybrid models which combine DeltaNet layers with (1) sliding-window attention layers every other layer or (2) two global attention layers, and find that these hybrids outperform strong transformer baselines.

==> figure/regbench.tex <==
\begin{wrapfigure}{l}{0.65\textwidth}
  \begin{center}
  \vspace{-7mm}
  \includegraphics[width=0.64\textwidth]{Styles/figure/regbench_all.pdf}
  \end{center}
    \vspace{-3mm}
  \caption{Accuracy (\%) on RegBench \cite{akyurek2024context}.}
  \vspace{-2mm}
\end{wrapfigure}

==> sections/discussion.tex <==

% \section{Generalizing Linear Transformers Beyond Elementwise Recurrence}
% To motivate our training algorithm, we first describe a generalization of  linear Transformers, of which DeltaNet, as well as  many models that will serve as baselines, are special cases.


Given a matrix-valued hidden state $\rmS_t \in \mathbb{R}^{d \times n}$ and current input $\vx \in \mathbb{R}^{d}$, we are interested in sequence models with the following form:
\begin{align*}
    &\rmS_t =   \rmS_{t-1} \bullet \rmM_t  + \vv_t  \vk_t^\intercal, && \text{(recurrence)} \\ &\vo_t = \rmS_t \vq_t,  && \text{(memory read-out)}
\end{align*}
where $\bullet$ is an associative operator (e.g., Hadamard product, matrix multiplication, etc.). The matrix $\rmM_t$ and vectors $\vv_t$, $\vk_t$, $\vq_t$  are (potentially non-linear) functions of the current input $\vx_t$. 

The use of an associative operator enables the use of parallel scan to calculate $\rmS_1, \dots, \rmS_L$ in $O(\log L)$ steps and $O(L)$ compute (ignoring the terms associated with the  associative operation)   if the inputs  $\vx_1, \dots, \vx_L$ are given. Hence, as long as the associative operator is not too expensive, training can be efficient. This model is also related to a variety of sequence models that have been previously explored: \textit{fast weights} \cite[][\textit{i.a.}]{hinton_using_1987,schmidhuber_learning_1992,ba_using_2016,schlag_linear_2021,irie_going_2021,mao_fine-tuning_2022},  \textit{state-space models} \cite[][\textit{i.a.}]{hasani2022liquid,fu_hungry_2023,mehta_long_2023,smith_simplified_2023,gu_mamba_2023}, and \textit{linear attention transformers} \cite[][\textit{i.a.}]{katharopoulos_transformers_2020,peng_random_2021,choromanski_rethinking_2021,sun2023retentive,pramanik_recurrent_2023,yang_gated_2023}. 

However,  parallel scan by itself is not sufficient for  training language models at practical scale due to  some associative operator's  being too expensive. Recent models such as such as Mamba \cite{gu_mamba_2023} and gated linear Transformers \cite{sun2023retentive,yang_gated_2023,qin_hgrn2_2024,peng_eagle_2024,beck2024xlstm}  thus make use of cheap element-wise recurrence updates, in particular the Hadamard product, i.e., $\bullet = \odot$. See Table~\ref{tab:overview} for how recent models can be cast into this form. 

Standard matrix multiplications (i.e., $\rmS_{t-1}\bullet \rmM_t = \rmS_{t-1}\rmM_t$) on the other hand can model richer  interactions  that go beyond elementwise recurrence. Without any structural assumptions on $\rmM_t$ however, these operations would take $O(dn^2)$  for each update (as opposed to $O(dn)$ for element-wise recurrences),  which would be prohibitively expensive. We thus consider a more restricted class of structured transformations, where the recurrence  is given by a diagonal plus low-rank (DPLR) matrix multiplication,
\begin{align*}
    \rmS_{t} = \rmS_{t-1}(\operatorname{diag}(\vd_t) + \va_t \vb_t^\intercal ) + \vv_t \vk_t^\intercal.
\end{align*}
It is easy to show that the DeltaNet is a special case of this ``DPLR Transformer'':
\begin{align*}
    \rmS_t &= \rmS_{t-1} -\vv_t^{\text{old}}\vk_t^\intercal+\vv_t^{\text{new} }\vk_t^\intercal\nonumber  =  \rmS_{t-1} + \beta_t \vv_t \vk_t^\intercal - \beta_t \left(\rmS_{t-1} \vk_t\right)\vk_t^\intercal = \rmS_{t-1} (\rmI - \beta_t \vk_t \vk_t^\intercal) + \beta_t \vv_t  \vk_t^\intercal.
    % \label{eq:delta_recurrent}
\end{align*}
The interpretation of the DeltaNet update as retrieving and updating values associated with a particular key (\S\ref{ssec:deltanet}) makes it an attractive parameterization for generalizing linear Transformers, which have been shown to struggle with in-context learning and retrieval \cite{}. And in preliminary experiments, we found little difference in performance between DeltaNet and the more general DPLR parameterzation. Hence, we adopt the  parameter-efficient DeltaNet parameterization for the rest of paper. However we emphasize that the hardware-efficient training algorithm described below---which is the core contribution of the present work---is applicable to the more general DPLR Transformer.

% While cheaper associative operators such as the Hadamard product (whose complexity is $O(dn)$) can enable FLOPs savings,  elementwise products cannot make use of specialized compute units (e.g., tensor cores) and are thus slow in practice; moreover, without any structural assumptions on $\rmM_{t}$ the hidden states $\rmS_{1},\dots,\rmS_{T}$ would need to be   either fully materialized and kept in memory (which would be impractical) or recomputed during backpropagation (which would be slow). Existing works such as Mamba \cite{gu_mamba_2023} Table~\ref{}) thus use a smaller expansion dimension $n$ to make sure that $\rmS_t$ is small enough to materialized only temporarily on faster memory.


\begin{table}[t!]
\footnotesize
\scalebox{0.87}{
\begin{tabular}{l ll}
\toprule
   Model  & Recurrence & Memory read-out \\
   \midrule
    Linear Attention \cite{katharopoulos_transformers_2020} &  $\rmS_t = \rmS_{t-1} + \vv_t  \vk_t^\intercal$ & $\vo_t = \rmS_t \vq_t $ \\
        \,\, + Kernel &  $\rmS_t = \rmS_{t-1} + \phi(\vv_t)  \vk_t^\intercal$ & $\vo_t = \rmS_t \phi(\vq_t) $ \\
\,\, + Normalization &  $\rmS_t = \rmS_{t-1} + \phi(\vv_t)  \vk_t^\intercal, \,\,\, \vz_t = \vz_{t-1} + \phi(\vk_t)$ & $\vo_t =  \rmS_t \phi(\vq_t) / (\vz_t^\intercal\phi(\vq_t))$  \\ 
    GLA \cite{yang_gated_2023,katsch_gateloop_2023}&  $\rmS_t =  \rmS_{t-1} \odot (\bbeta_t \balpha_t^\intercal) + \vv_t  \vk_t^\intercal$ & $\vo_t = \rmS_t \vq_t$  \\
       HGRN2 \cite{qin_hgrn2_2024} &  $\rmS_t =   \rmS_{t-1} \odot (\balpha_t  \mathbf{1}^\intercal) + \vv_t  (\mathbf{1} - \balpha_t)^\intercal $ & $\vo_t = \rmS_t \vq_t$  \\   
    RWKV-6 \cite{peng_eagle_2024} &  $\rmS_t =   \rmS_{t-1} \odot (\balpha_t  \mathbf{1}^\intercal) + \vv_t  \vk_t^\intercal $ & $\vo_t = (\rmS_{t-1} + (\vd \odot  \vv_t ) \vk_t^\intercal) \vq_t$  \\    
    Mamba \cite{gu_mamba_2023} & $\rmS_t = \rmS_{t-1} \odot \exp(-(\balpha_t \mathbf{1}^\intercal)\odot \exp(\mA)) + (\balpha_t \odot \vx_t) \vk_t^\intercal $ & $\vo_t = \rmS_t \vq_t + \vd \odot \vx_t$  \\
    mLSTM  \cite{beck2024xlstm} &$\rmS_t = f_t \rmS_{t-1} + i_t \vv_t  \vk_t^\intercal, \,\,\, \vz_t = f_t \vz_{t-1} + i_t \vk_t$ & $\vo_t = \rmS_t \vq_t / \max\{1, |\vz_t^\intercal \vq_t |\}$  \\
    DeltaNet \cite{schlag_linear_2021}& $\rmS_t =  \rmS_{t-1} (\mathbf{I} - \beta_t \vk_t \vk_t^\intercal) + \beta_t \vv_t  \vk_t^\intercal$ & $\vo_t = \rmS_t \vq_t$ \\
     % Linear DPLR Transformer &    $ \rmS_{t} = \rmS_{t-1}(\operatorname{diag}(\vc_t) + \va_t \vb_t^\intercal ) + \vv_t \vk_t^\intercal$  & $\vo_t = \rmS_t \vq_t$ \\
    \bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{Overview of recent linear Transformer models, which make use of a matrix-valued hidden state $\rmS_{t} \in \mathbb{R}^{d\times n}$ that is updated through an associative recurrence followed by an outer-product-based addition. Some models make use of an additional linear RNN with hidden state vector $\vz_t$, which used to normalized the query vector $\vq_t$. Variables with the subscript $t$ ($\vv_t, \vk_t, \vq_t, \balpha_t, \bbeta_t, \va_t, \vb_t, \vc_t, f_t, i_t$) are (potentially non-linear) functions of the current input $\vx_t$. Non-time-varying (learned) parameters ($\mA$, $\vd$) are denoted without subscripts.}
\label{tab:overview}
\end{table}



==> tables/kernel.tex <==
\begin{wraptable}{r}{0.43\textwidth}
%\begin{table}
\vspace{-5mm}
\centering
\small 
        \begin{tabular}{rcr}
        \toprule[0.5mm]
     $L$  & $d_{\text{head}}$ &  Speed-up \\
      \bottomrule
2048 &  64 & 5.5x \\
4096 &  64 & 7.6x \\
8192 &  64 & 11.5x \\ 
2048 & 128 & 8.9x \\
4096 & 128 & 13.2x \\
2048 & 256 & 13.7x \\
        \bottomrule
        \end{tabular}
    % \vspace{-2mm}
\caption{Speed comparison between the recurrent and chunkwise algorithms for DeltaNet on a single H100 GPU. }
\label{tab:kernel_speed}
% \end{table}
%\end{table}
\vspace{-8mm}
\end{wraptable}


